DaLC: Domain Adaptation Learning Curve Prediction for Neural Machine Translation

Domain Adaptation (DA) of Neural Machine Translation (NMT) model often relies on a pre-trained general NMT model which is adapted to the new domain on a sample of in-domain parallel data. Without parallel data, there is no way to estimate the potential benefit of DA, nor the amount of parallel samples it would require. It is however a desirable functionality that could help MT practitioners to make an informed decision before investing resources in dataset creation. We propose a Domain adaptation Learning Curve prediction (DaLC) model that predicts prospective DA performance based on in-domain monolingual samples in the source language. Our model relies on the NMT encoder representations combined with various instance and corpus-level features. We demonstrate that instance-level is better able to distinguish between different domains compared to corpus-level frameworks proposed in previous studies. Finally, we perform in-depth analyses of the results highlighting the limitations of our approach, and provide directions for future research.

==> features.tex <==
\tbr{
\subsection{Features}
Our main purpose of featurization is extracting and modeling the \textit{domain difficulty} from the input sentence $x_i$ and the source-side of in-domain corpus  $D_{in}^{s}$. We defines \textit{domain difficulty} as the two levels : (1) instance-level and (2) corpus-level. 

The instance level features mainly encodes how much distinct the input sentence from $D_{out}$, which the model saw in the pre-training steps. As mentioned in Section 5.2, we basically utilize the baseline NMT encoder representations as the one of instance-level features. Additionally, we hypothesize the pre-trained model is hard to generate the distinct sentence rather than the similar sentence to $D_out$. Inspired from uncertainty scores of Active learning, we utilize the four difficulties as the our instance-level features, where the difficulties comes from the pre-trained NMT model with the input. 


The particularity of Domain Adaptation task is that we usually start from the baseline NMT model (in what follows referred to as \textit{baseline}) which is  adapted to a domain of interest with relatively small amount of data. We believe that the representations provided by baseline model could contain a lot information relative to the domain adaptation capacity of each particular domain. Thus, we could imagine, that "easier" domains could be distinguished from "harder" domains based on NMT encoder representations. 


\noindent\textbf{Normalized probability (np)} computes the probability  from the input sentence, 
\begin{equation}\label{eqn:np_feature}equation -probablity,\end{equation}

where $y*=(y_{1}...y_{m})$ indicates the generated sentence from the pre-trained model and $P(y_i |M_{\theta},x,y_{<i})$ is a probability distribution of the whole vocabulary at the $i$-th generate step. If this score is low, this input sentence is hard to translate by the pre-trained model.  


\noindent\textbf{Margin score (ms)} is obtained from  the difference between the most high probability score word and the second high probability score at each decoding step, 
\begin{equation}\label{eqn:margin_feature}equation2 -probablity,\end{equation}
where $y^1_{i}$ and $y^2_{i}$ represent the most high score word and the second high score word, respectively.
Compared to normalized probability, this score considers how much confidence the most high probability score words is at each decoding step. The low confidence of the translated sentence means the model fail to capture the context of the input sentence, because the model is not familiar with the input. 


\noindent\textbf{Total token entropy score (tes)} is the cross-entropy value on the all probability distribution of generated tokens,
\begin{equation}\label{eqn:total_entropy}equation3 -probablity,\end{equation}
. This score considers all tokens in vocabulary, rather than only the most high token. If the probability distribution of the token were uniform, the model confuse to choose the next word. It means the pre-train model suffers from the domain-shift problem. 


\noindent\textbf{Average token entropy scrore (aes)} is normalized the total token entropy by the length of the generated sentence. 


\noindent\textbf{BERT score (bs)} is the well known metric for measuring the semantically the same between the input sentence and its generate sentence[need cite].
%This score is computed without the reference sentence.
It is feasible to compute the score in our setting, because this score does not need to the reference sentence. Moreover, it is good evident for the model to figure out the initial translation quality before the fine-tuning with the sampled $D_{in}$ corpus. 

To capture the features for the sampled trained $D_{in}$ dataset, we extract the corpus-level features the only-source language. Note that this features shared across the instances, which is assumed in the same sampled in-domain corpus. Main purpose of the corpus-level features quantify the new information, which is the model is able to learn from the sampled in-domain dataset $D_{in}$.Aforementioned in Section XX,the performance of the fine-tuned model with $D_{in}$ is very different from the characteristic of the domain and the sampled fine-tuned dataset $D_{in}$. 


\noindent\textbf{Vocabulary overlap} is the overlap ratio between the pre-train vocabulary and the sampled in-domain vocabulary,  ,
\begin{equation}\label{eqn:total_entropy}equation4,\end{equation}
where ~~ xx . It represents the corpus-level similarity between two corpus based on the vocabularies of each corpus. This 


\noindent\textbf{Type token ratio} 


\noindent\textbf{Number of sentences} indicates the number of sentences in the sampled $D_in^{s}$. 
\noindent\textbf{Number of tokens} 

\noindent\textbf{Vocabulary size} is the number of the unique words in the sampled $D_in^{s}$, where the unique words extracted from the raw sentence before applying in the byte-pair encoding. 

}
